Efficient Black-box Checking of Snapshot Isolation in Databases

Snapshot isolation (SI) is a prevalent weak isolation level that avoids the performance penalty imposed by serializability and simultaneously prevents various undesired data anomalies. Nevertheless, SI anomalies have recently been found in production cloud databases that claim to provide the SI guarantee. Given the complex and often unavailable internals of such databases, a black-box SI checker is highly desirable. In this paper we present PolySI, a novel black-box checker that efficiently checks SI and provides understandable counterexamples upon detecting violations. PolySI builds on a novel characterization of SI using generalized polygraphs (GPs), for which we establish its soundness and completeness. PolySI employs an SMT solver and also accelerates SMT solving by utilizing the compact constraint encoding of GPs and domain-specific optimizations for pruning constraints. As demonstrated by our extensive assessment, PolySI successfully reproduces all of 2477 known SI anomalies, detects novel SI violations in three production cloud databases, identifies their causes, outperforms the state-of-the-art black-box checkers under a wide range of workloads, and can scale up to large-sized workloads.

==> algs/backup.tex <==
% backup.tex


  % collect WW edges and RW edges in constraints
    % \ForAll{$\tuple{\eithervar, \orvar} \in \cons_{\g}$}
    %   \label{line:encodeconstraints-forall-cons-composition}
    %   \ForAll{$\edgevar \gets (\_, \_, \typevar) \in \eithervar \cup \orvar$}
    %     \If{$\typevar = \WW$}
    %       \State $\edges_{A} \gets @ \cup \set{\edgevar}$
    %     \Else
    %       \State $\edges_{B} \gets @ \cup \set{\edgevar}$
    %     \EndIf
    %   \EndFor
    % \EndFor

  % encodeconstraints by Chen
  \Function{\encodeconstraints}{\null} \Comment{\red{by Chen}}
    \State $GraphA, GraphB \gets$ Graph\{all transactions, \{\}\}
    \State $L_{true} \gets \{\}$

    \For{$e$ in $KnownGraph$.\{SO $\cup$ WR $\cup$ WW\}}
      \State $l \gets$ Literal\{\}
      \State $GraphA \pluseq$ ($e$, l)
      \State $L_{true} \pluseq l$
    \EndFor

    \For{$e$ in $KnownGraph$.RW}
      \State $l \gets$ Literal\{\}
      \State $GraphB \pluseq$ ($e$, l)
      \State $L_{true} \pluseq l$
    \EndFor

    \For{($E_{1}$, $E_{2}$) in $constraints$}
      \State $l_{1all} \gets$ true
      \State $l_{1none} \gets$ true
      \State $l_{2all} \gets$ true
      \State $l_{2none} \gets$ true
      \For{$e$ in $E_{1}$}
        \State $l \gets$ Literal\{\}
        \State $l_{1all} \gets l_{1all} \wedge l$
        \State $l_{1none} \gets l_{1none} \wedge \neg l$
        \If{$e$ is WW}
          \State \red{$GraphA$ $\pluseq$ ($tx1$, $tx2$, l)}
        \Else
          \State \red{$GraphB$ $\pluseq$ ($tx1$, $tx2$, l)}
        \EndIf
      \EndFor
      \For{$e$ in $E_{2}$}
        \State $l \gets$ Literal\{\}
        \State $l_{2all} \gets l_{2all} \wedge l$
        \State $l_{2none} \gets l_{2none} \wedge \neg l$
        \If{$e$ is WW}
          \State $GraphA$ $\pluseq$ ($tx1$, $tx2$, l)
        \Else
          \State $GraphB$ $\pluseq$ ($tx1$, $tx2$, l)
        \EndIf
      \EndFor
      \State $L_{true} \pluseq (l_{1all} \wedge l_{2none}) \vee (l_{1none} \wedge l_{2all})$
    \EndFor

    \State $GraphC \gets GraphA$
    \For{$tx1$ in $GraphA$}
      \For{($tx2$, $l_{1}$) in \Call{InEdges}{$graphA$, $tx1$}}
        \For{($tx3$, $l_{2}$) in \Call{OutEdges}{$graphB$, $tx1$}}
          \State $graphC$ $\pluseq$ ($tx2$, $tx3$, $l_{1} \wedge l_{2}$)
        \EndFor
      \EndFor
    \EndFor
    \State \Return $(L_{true}, GraphC)$
  \EndFunction

==> algs/clip-counterexample.tex <==
%clip-counterexample.tex

\begin{algorithm}[t]
	\caption{Algs of clip counterexample}
	\label{alg:counterexample}
	\begin{algorithmic}[1]
		\Statex ${\cycle}_1 = (\V, \E)$: the first cycle to clip
		\Statex ${\cycle}_2 = (\V, \E)$: the second cycle to clip, (if ${\cycle}_2$ exists)
		\Statex $\H = (\V, \E)$: the history in which ${\cycle}_1$ and ${\cycle}_2$ are found
		
		\Statex
        \Procedure{\ClipCounterexample}{${\cycle}_1$,${\cycle_2}$,$\H$}
            \State 
                $\Call{\SoCutCycle}{{\cycle}_1}$
            \State 
                $\Call{\SoMergeTxn}{{\cycle}_1}$
            \State 
                $\Call{\SoCutCycle}{{\cycle}_2}$
            \State 
                $\Call{\SoMergeTxn}{{\cycle}_2}$
            \State 
                $counterexample$ $\gets$ $\Call{\Restore}{{\cycle}_1,{\cycle}_2,\H}$
            \State
                \Return $counterexample$
        \EndProcedure
		
		\Statex
        \Procedure{\SoCutCycle}{$\cycle$}
            \ForAll{$u \in \cycle.\V$}
                \ForAll{$v \in \cycle.\V-\{u\}$ such that $u,v$ are not adjacent}
                    \If{$u\rel{so}v$ }
                        \State
                            $\cycle$ $\gets$ $P_{\cycle}(v->u) + u\rel{so}v$
                        \State
                            \Comment{$P_{\cycle}(v->u)$ means the path from $v$ to $u$ in $\cycle$}
                    \EndIf
                    \If{$v\rel{so}u$ }
                        \State
                            $\cycle$ $\gets$ $P_{\cycle}(u->v) + v\rel{so}u$
                    \EndIf
                \EndFor
            \EndFor
        \EndProcedure
        
        \Statex
        \Procedure{\SoMergeTxn}{$\cycle$}
            \ForAll{$u \in \cycle.\V$}
                \If{$u\rel{so}v$ exists in $\cycle$ }
                    \State
                        $t$ $\gets$ $u$ $\cup$ $v$
                    \State
                        \Comment{$ops$ $\in$ $u$ $\rel{po}$ $ops$ $\in$ $v$ in $t$}
                \EndIf
            \EndFor
        \EndProcedure
        
        \Statex
        \Procedure{\Restore}{$\cycle_1$,$\cycle_2$,$\H$}
            \ForAll{$u \in \cycle_1.\V$ and $v \in \cycle_2.\V$}
                \State
                    $Counterexample$ $\gets$ $\cycle_1$ $\cup$ $\cycle_2$
                \If{$u\rel{wr}v$ exists in $\H$ }
                    \State
                        $Counterexample$ $\gets$ $Counterexample$ $\cup$ $u\rel{wr}v$
                \EndIf
                \If{$v\rel{wr}u$ exists in $\H$ }
                    \State
                        $Counterexample$ $\gets$ $Counterexample$ $\cup$ $v\rel{wr}u$
                \EndIf
            \EndFor
            \State
            \Return $Counterexample$
        \EndProcedure
	\end{algorithmic}
\end{algorithm}


==> algs/incremental.tex <==
% incremental.tex

\begin{algorithm}[t]
	\caption{Algs of OOPSLA(testing SI)}
	\label{OOPSLA_TEST_SI}
	\begin{algorithmic}[1]
		\Statex
		\CheckSI[$(\textbf{history} \quad h, \qquad \textbf{prefix} \quad T')$]
		\If{h.T == T'}{ \Return true \;} \EndIf
		\For{$\forall t \in h.T, s.t. \forall t'\in T', <t,t'> \notin wr \cup so$}
		{
			\If{$T' \ntriangleright T' \biguplus \{t\}$}{ continue }
			\EndIf
			\If{$T' \biguplus \{t\} \notin seen \wedge {\sf CheckSER}(h, T' \biguplus \{t\}) $}{ \Return true }
			\EndIf \\
			\hspace{28pt} $seen \leftarrow seen \cup \{(T' \biguplus \{t\})\}$
		}
		\EndFor
		\EndCheckSI
		\\
		\algorithmiccomment{$T \biguplus \{t\}:1.\{t'|t' \in T/T' \wedge t' \rel{wr/so} t \} = \phi $} \\
		\algorithmiccomment{2.$t$ writes $y$ $\Rightarrow \{t'|t' \in T/T' \wedge (\exists z, s.t. $ $t,t'$ reads $z$ $, ver(z)_t > ver(z)_{t'}) \wedge (\exists t''\in T', t'' \rel{wr_y} t')\} = \phi$}
		\\
	\end{algorithmic}
\end{algorithm}

==> figs/banking.tex <==
% banking.tex

\begin{figure}[t]
  \centering
  \includegraphics[width = 0.40\textwidth]{figs/banking-lostupdate}
  \caption{A banking example illustrating a \emph{lost update} anomaly that is disallowed by \si.
	We omit the transaction that writes the initial value \$$0$ of $\acct$.
	The labeled edges are explained in Example~\ref{ex:depgraph-si}.}
  \label{fig:banking}
\end{figure}

==> figs/ce-dgraph.tex <==
% ce-dgraph.tex

%\begin{figure*}[t]
%  \centering
%  \begin{subfigure}[c]{0.36\textwidth}
% %   \centering
%    \includegraphics[width = 1.00\textwidth]{figs/ce}
%    \caption{\red{The original counterexample.}}
%    \label{fig:ce}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[c]{0.35\textwidth}
%%    \centering
%    \includegraphics[width = 1.00\textwidth]{figs/ce-so-two}
%    \caption{\red{The counterexample after $\dots$}.}
%    \label{fig:ce-so-two}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[c]{0.28\textwidth}
%%    \centering
%    \includegraphics[width = 1.00\textwidth]{figs/ce-so-one}
%    \caption{\red{The counterexample after $\dots$}.}
%    \label{fig:ce-so-one}
%  \end{subfigure}
%  \caption{Illustration of an \si{} violation found in Dgraph.
%    The pair $(10, 471)$ represents the 471st transaction on the 10th session.
%    The $\SO$ and $\WR$ relations are represented by solid arrows.
%    The $\WW$ and $\RW$ relations are represented by dashed arrows and dotted arrows, respectively.}
%  \label{fig:ce-dgraph}
%\end{figure*}

==> figs/dgraph-ce-complete.tex <==
% dgraph-ce-complete.tex

\begin{figure*}[t]
  \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width = \textwidth]{figs/color/DGraph_counter_example_original}
        \caption{Original output}
		\label{fig:dgraph-ce-complete-original}
    \end{subfigure}\hspace{10ex}
 %   \hill
    \begin{subfigure}[b]{0.38\textwidth}
        \centering
        \includegraphics[width = 1.25\textwidth]{figs/color/DGraph_counter_example_recovery_step1}
        \caption{Missing participants}
		\label{fig:dgraph-ce-complete-participants}
    \end{subfigure}\vspace{2ex}
 %   \hfill
    \begin{subfigure}[b]{0.38\textwidth}
        \centering
        \includegraphics[width = 1.25\textwidth]{figs/color/DGraph_counter_example_recovery_step2}
        \caption{Recovered scenario}
		\label{fig:dgraph-ce-complete-recovered}
    \end{subfigure}\hspace{15ex}
  %  \hfill
    \begin{subfigure}[b]{0.38\textwidth}
        \centering
        \includegraphics[width = 1.25\textwidth]{figs/color/DGraph_counter_example_delete}
        \caption{Finalized scenario}
		\label{fig:dgraph-ce-complete-finalized}
    \end{subfigure}
    \caption{Causality violation: the SI anomaly found in Dgraph.
     Dashed and solid  arrows represent uncertain and  certain dependencies, respectively.
     Recovered transactions are colored in green.
     The core dependencies involved in the two sub-scenarios are colored in red and blue, respectively.}
   \label{fig:dgraph-ce-complete}
\end{figure*}

==> figs/fig-int-axiom.tex <==
% fig-int-axiom.tex

\begin{figure*}[t]
  \centering
  \begin{mdframed}
	  \begin{align}
		&\forall (\E, \po) \in \h.\;
		  \forall \evar \in \Event.\;
		    \forall \keyxvar, \valvar.\;
			  \big(\op(\evar) = \readevent(\keyxvar, \valvar)
			  \land \set{\fvar \mid \op(\fvar) = \_(\keyxvar, \_) \land \fvar \rel{\po} \evar} \neq \emptyset\big) \nonumber \\
			  &\quad \implies \op(\max_{\po} \set{\fvar \mid \op(\fvar) = \_(\keyxvar, \_) \land \fvar \rel{\po} \evar}) = \_(\keyxvar, \valvar)
          \tag{\intaxiom} \label{eq:intaxiom}
    \end{align}
  \end{mdframed}
\end{figure*}
  % \caption*{The \intaxiom{} axiom (from~\protect\cite{AnalysingSI:JACM2018}).}
  % \label{fig:int-axiom}

==> figs/int-axiom.tex <==
% int-axiom.tex
\begin{align}
  &\forall (\E, \po) \in \h.\;
   \forall \evar \in \Event.\;
   \forall \keyxvar, \valvar.\; \tag{\intaxiom} \label{eq:intaxiom} \\
	&\quad \big(\op(\evar) = \readevent(\keyxvar, \valvar)
	\land \set{\fvar \mid \op(\fvar) = \_(\keyxvar, \_) \land \fvar \rel{\po} \evar} \neq \emptyset\big) \nonumber \\
	&\qquad \implies \op(\max_{\po} \set{\fvar \mid \op(\fvar) = \_(\keyxvar, \_) \land \fvar \rel{\po} \evar}) = \_(\keyxvar, \valvar) \nonumber
\end{align}

==> figs/polygraph_changed.tex <==
% polygraph.tex

\begin{figure}[h]
  \centering
  \begin{subfigure}[c]{0.23\textwidth}
    \centering
    \includegraphics[width = 1.00\textwidth]{figs/polygraph_changed}
    \caption{changed}
    %\label{fig:polygraph}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.23\textwidth}
    \centering
    \includegraphics[width = 1.00\textwidth]{figs/g-polygraph_changed}
    \caption{changed}
    %\label{fig:g-polygraph}
  \end{subfigure}
  \caption{changed figure 3}
  %\label{fig:polygraph-g-polygraph}
\end{figure}

==> figs/pruning-cases-wrapfig.tex <==
% pruning-cases-wrapfig.tex

\begin{wrapfigure}{t}{0.18\textwidth}
%\vspace{-2ex}
  \begin{subfigure}[c]{0.17\textwidth}
    \centering
    \includegraphics[width = 0.95\textwidth]{figs/pruning-ww-case}
    \caption{$\WW$ edge $(\fromvar, \tovar)$}
   \label{fig:pruning-ww-case}
   \vspace{2ex}
  \end{subfigure}
  \begin{subfigure}[c]{0.17\textwidth}
    \centering
    \includegraphics[width = 0.90\textwidth]{figs/pruning-rw-case}
    \caption{$\RW$ edge $(\fromvar, \tovar)$ }
   \label{fig:pruning-rw-case}
  \end{subfigure}
  \caption{Two cases for pruning constraints.}
  \label{fig:pruning}
  %  \vspace{-2ex}
\end{wrapfigure}

==> figs/pruning-cases_changed.tex <==
% pruning-cases.tex

\begin{figure}[t]
  \centering
  \begin{subfigure}[c]{0.23\textwidth}
    \centering
    \includegraphics[width = 0.75\textwidth]{figs/pruning-ww-case}
    \caption{$(\fromvar, \tovar)$ is a $\WW$ edge.}
    \label{fig:pruning-ww-case}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.23\textwidth}
    \centering
    \includegraphics[width = 0.80\textwidth]{figs/pruning-rw-case}
    \caption{$(\fromvar, \tovar)$ is an $\RW$ edge.}
    \label{fig:pruning-rw-case}
  \end{subfigure}
  \caption{Two cases in pruning constraints.}
\end{figure}

==> figs/pruning-example.tex <==
% pruning-example.tex

\begin{figure*}[t]
  \centering
%  \begin{subfigure}[c]{0.23\textwidth}
%    \centering
 %   \includegraphics[width = 1.00\textwidth]{figs/pruning}
 %   \caption{The history with $\SO$ and $\WR$ relations.}
%    \label{fig:pruning-history}
%  \end{subfigure}
%  \hfill
  \begin{subfigure}[c]{0.28\textwidth}
 %   \centering
    \includegraphics[width = 1.00\textwidth]{figs/pruning-ww}
    \caption{$T_{2} \rel{\WW(\keyxvar)} T_{1}$ is pruned
      due to the cycle $T_{2} \rel{\WW(\keyxvar)} T_{1} \rel{\SO/\WR(\keyyvar)} T_{2}$.}
    \label{fig:pruning-ww}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.28\textwidth}
%    \centering
    \includegraphics[width = 1.00\textwidth]{figs/pruning-rw-either}
    \caption{$T_{3} \rel{\WW(\keyyvar)} T_{1}$ is pruned
      due to the cycle $T_{4} \rel{\RW(\keyyvar)} T_{1} \rel{\WR(\keyxvar)} T_{4}$.}
    \label{fig:pruning-rw-either}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.28\textwidth}
%    \centering
    \includegraphics[width = 1.00\textwidth]{figs/pruning-rw-or}
    \caption{$T_{1} \rel{\WW(\keyyvar)} T_{3}$  stays as  cycle $T_{4} \rel{\RW(\keyxvar)} T_{2} \rel{\RW(\keyyvar)} T_{3} \rel{\WR(\keyyvar)} T_{4}$
      is allowed by \si.}
    \label{fig:pruning-rw-or}
  \end{subfigure}
  \caption{Illustration of pruning constraints.
     $\SO$ and $\WR$ relations are represented by solid arrows.
     $\WW$ and $\RW$ relations are represented by dashed arrows and dotted arrows, respectively.}
  \label{fig:pruning-example}
\end{figure*}

==> figs/pruning-example_changed.tex <==
% pruning-example.tex

\begin{figure*}[h]
  \centering
%  \begin{subfigure}[c]{0.23\textwidth}
%    \centering
 %   \includegraphics[width = 1.00\textwidth]{figs/pruning}
 %   \caption{The history with $\SO$ and $\WR$ relations.}
%    \label{fig:pruning-history}
%  \end{subfigure}
%  \hfill
  \begin{subfigure}[c]{0.31\textwidth}
 %   \centering
    \includegraphics[width = 1.00\textwidth]{figs/pruning-ww_changed}
    \caption{changed}
    %\label{fig:pruning-ww}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.31\textwidth}
%    \centering
    \includegraphics[width = 1.00\textwidth]{figs/pruning-rw-either_changed}
    \caption{changed}
    %\label{fig:pruning-rw-either}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.31\textwidth}
%    \centering
    \includegraphics[width = 1.00\textwidth]{figs/pruning-rw-or_changed}
    \caption{changed.}
    %\label{fig:pruning-rw-or}
  \end{subfigure}
  \caption{Changed figure 5}
  \label{fig:pruning-example-color}
\end{figure*}

==> figs/si-examples.tex <==
% si-examples.tex

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.18\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figs/post-comment}
    \caption{%A social media example illustrating a 
 Causality violation.}
  %  \label{fig:post-comment}
  \end{subfigure}\hspace{4ex}
  %\hfill
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figs/banking-lostupdate}
    \caption{%A banking example illustrating a
Lost update.}
  %  \label{fig:banking}
  \end{subfigure}
  \caption{\label{si-examples} Anomalies disallowed by \si.
  We omit the initial transactions.
    The labeled arrows are explained in Section~\ref{ss:si-formal}.}
\end{figure}

==> figs/si-examples_changed.tex <==
% si-examples.tex

\begin{figure}[h]
  \centering
  \begin{subfigure}[c]{0.18\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figs/post-comment}
    \caption{Not changed}
    %\label{fig:post-comment}
  \end{subfigure}\hspace{4ex}
  %\hfill
  \begin{subfigure}[c]{0.23\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figs/banking-lostupdate_changed}
    \caption{changed}
    \label{fig:banking}
  \end{subfigure}
  \caption{changed figure 1}
  %\label{fig:polygraph-g-polygraph}
\end{figure}

==> figs/tcm-more.tex <==
% tcm-more.tex

\begin{figure}[t]
  \centering
%  \begin{tikzpicture}[model/.style = {draw, minimum size = 15pt},
%    node distance = 0.5cm and 1.5cm]
%
%    \node[model] (rc) {\textsc{RC}};
%    \node[model, right = of rc] (cs) {\textsc{CS}};
%    \node[model, right = of cs] (rr) {\textsc{RR}};
%    \node[model, right = of rr] (ser) {\textsc{SER}};
%
%    \node[model, below = of rc] (ci) {\textsc{CI}};
%    \node[model, right = of ci] (ra) {\textsc{RA}};
%    \node[model, right = of ra] (psi) {\textsc{PSI}};
%    \node[model, below = of psi] (pc) {\textsc{PC}};
%    \node[model, right = of psi] (si) {\textsc{SI}};
%
%    \path[every edge, ->, thick] (rc) edge (cs) edge (ra)
%       (cs) edge (rr)
%       (rr) edge (ser)
%       (ci) edge (ra)
%       (ra) edge (psi) edge (pc)
%       (pc) edge (si)
%       (psi) edge (si)
%       (si) edge (ser);
%  \end{tikzpicture}
  \includegraphics[scale=0.48]{figs/hierarchy.pdf}
  \caption{A hierarchy of database isolation levels.
  $A \rightarrow B$: $A$ is strictly weaker than $B$.
  CI: cut isolation~\cite{HAT:VLDB2013};
  RC: read committed~\cite{CritiqueANSI:SIGMOD1995};
  RA: read atomicity~\cite{RAMP:TODS2016};
  RR: repeatable read~\cite{Adya:PhDThesis1999};
  TCC: transactional causal consistency~\cite{Eiger:NSDI2013};
  PSI: parallel snapshot isolation~\cite{PSI:SOSP2011};
  %PC: prefix consistency~\cite{pc};
  SI: snapshot isolation~\cite{AnalysingSI:JACM2018}; %CritiqueANSI:SIGMOD1995,LazyReplSI:VLDB2006,
  S: serializability~\cite{CritiqueANSI:SIGMOD1995}.}
  \label{fig:hierarchy}
\end{figure}

==> figs/tcm.tex <==
% tcm.tex

\begin{figure}[t]
  \centering
  \begin{tikzpicture}[model/.style = {draw, minimum size = 10pt},
    edge/.style = {->, thick},
    node distance = 0.1cm and 1.0cm]

    \node[model] (ra) {\textsc{RA}};
    \node[model, above left = of ra] (rc) {\textsc{RC}};
    \node[model, below left = of ra] (ci) {\textsc{CI}};

    \node[model, above right = of ra] (psi) {\textsc{PSI}};
    \node[model, below right = of ra] (pc) {\textsc{PC}};

    \node[model, below right = of psi] (si) {\textsc{SI}};
    \node[model, right = of si] (ser) {\textsc{SER}};

    \draw[edge] (rc) to (ra);
    \draw[edge] (ci) to (ra);
    \draw[edge] (ra) to (psi);
    \draw[edge] (ra) to (pc);
    \draw[edge] (psi) to (si);
    \draw[edge] (pc) to (si);
    \draw[edge] (si) to (ser);
  \end{tikzpicture}
  \caption{A hierarchy of database isolation levels.
  $A \rightarrow B$: $A$ is strictly weaker than $B$.
  RC: read committed~\cite{CritiqueANSI:SIGMOD1995};
  CI: cut isolation~\cite{HAT:VLDB2013};
  RA: read atomicity~\cite{ra};
  PC: prefix consistency~\cite{pc};
  PSI: parallel snapshot isolation~\cite{PSI:SOSP2011};
  SI: snapshot isolation~\cite{AnalysingSI:JACM2018}; %CritiqueANSI:SIGMOD1995,LazyReplSI:VLDB2006,
  SER: serializability~\cite{CritiqueANSI:SIGMOD1995}.}
  \label{fig:hierarchy}
\end{figure}

==> sections/Informative.tex <==
% Informative.tex

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Informative} \label{ss:informative}

MonoSAT will output a cycle 
when it finds a violation of SI from the input history.
However, we can hardly identify 
which kinds of violation is the main reason that leads to the cycle.
The main reason for this is that 
though a violation will lead to a cycle, 
the cycle itself does not contain all the information of that violation.
Thus, we propose an algorithm
which can recover the information of the violation.
We will briefly introduce it in this section.
Our algorithm can be divided into three steps, 
corresponding to the three strategies we use.

1). We can use the $RW$ dependencies to recover
useful information. 
A $RW$ dependency must be associated with a $WW$ dependency 
and a $WR$ dependency. 
Thus, we can check all the $RW$ dependencies in the output cycle 
and recover the related $WW$ and $WR$ dependencies.

2). In the output cycle, there may be several
edges which are in constraints rather than 
in known graph.
And we call the set of those dependencies $DC$.
In a constraint, there are two sets of dependencies, 
representing two different possibilities.
For any dependency $dp_1 \in DC$, 
we find its opposite dependency $dp_2$ in the same
constraint.
$dp_2$ must be in another cycle, then we recover 
this cycle.

Now we have recover all the information associated
the violation which leads to the output cycle.
But the graph we got may be huge, so we need to
delete some redundant information. And this is step 3.

3). We tag all the `deterministic' dependencies 
and delete others.
Here `deterministic' means the dependencies 
must exist when the history is input.
We judge these dependencies are deterministic:
(a). dependencies in known graph ($SO$ and $WR$).
(b). In a cycle, 
if there is only one dependency $dp_1$ that is not deterministic, 
then the opposite dependency $dp_2$ which is in the same
constraint with $dp_1$ is deterministic.

After doing the 3 steps, we can identify the violation
much easier.
Here we give 2 examples.
First is the violation we found in Galera.
(Figure~\ref{informative-galera})
In this figure, the first picture is the original output we got.
Then we perform two steps, we got the second picture, 
which has the complete information of the violation.
But the number of dependencies is too large so we perform step 3.
Then we get the last picture, 
which can trivially tell us this is a `lost update'.
The second example is the violation we found in Dgraph.(figure~\ref{informative-DGaph}).
The original output is a cycle of 3 transactions 
and it is impossible to identify the violation just from the cycle.
After our 3-step algorithm we get a mo complex picture,
which can tell us this is a `violation of causality'.
(Transaction (9,428) do not read $key_{656}$ from transaction (10,472), and there is a causal dependency from (10,472) to (9,428)).


\begin{figure*}
    \centering
    \includegraphics[scale=0.3]{figs/galera_counter_example.pdf}
    \caption{Lost update: the SI violation found in MariaDB-Galera.  \red{Explain }}
    \label{informative-galera}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.3]{figs/Dgraph_counter_example.pdf}
    \caption{Causality violation: the SI anomaly found in Dgraph. \red{Explain }}
    \label{informative-dgraph}
\end{figure*}



==> sections/impl.tex <==
% impl.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Implementation}  \label{section:impl}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/incremental.tex <==
% incremental.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{An Incremental Checking Algorithm} \label{sss:incremental}
\nobi{We could summarize the idea when we introduce the competitor and refer to Appendix for all these details}
\cite{Complexity:OOPSLA2019} gives an incremental checking alg for SER, and it can be simply modified for checking SI. The input is a history $h$ and a prefix $T$ of $h$. Assume that the prefix has been checked by recursive function, what need to be done is add a Txn $t$ $\in$ $h/T$ to $T$ and extend the prefix. The difficulty is how to pick $t$ so that $T+{t}$ does not violate SI. And we believe that $t$ which satisfies the following two conditions is suitable:

1. $\{t_y | t_y \in h/T \wedge t_y \rel{wr/so} t\} = \phi$

2. If $t$ writes $x$, then $\{t_y| t_y \in h/T \wedge (\exists z, st t, t_y reads z, ver(z)_{t_y} > ver(z)_t) \wedge (\exists t_x \in T, t_x \rightarrow t_y)\} = \phi$

We can check all the Txn in $h/T$ and select a suitable $t$ one by one.

\todohuang{describe the incremental checking algorithm for SI based on~\cite{Complexity:OOPSLA2019}}

\input{algs/incremental}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/intro.tex <==
% intro.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}  \label{section:intro}

\bfit{Transactions and Isolation Levels.}
ACID transactions provide an ``all-or-none'' abstraction
and isolate concurrent computations on shared data from each other~\cite{Bernstein:Book1986}.
This greatly simplifies client programming, and programmers prefer to strong isolation levels.
The gold standard for isolation is {\it serializability} (\ser)~\cite{SER:JACM1979,Bernstein:Book1986},
which ensures that all transactions appear to execute serially, one after another.
Unfortunately, ensuring \ser, particularly in a distributed setting, is inevitably expensive~\cite{HAT:VLDB2013}.
Therefore, many databases choose to implement weaker isolation levels.

\bfit{Snapshot Isolation (SI).}
Snapshot isolation (\si)~\cite{CritiqueANSI:SIGMOD1995} is one of the most popular weak isolation levels,
implemented by both classic centralized databases like Microsoft SQL Server~\cite{SQLServer} and Oracle Database~\cite{Oracle}
and emerging distributed databases like Google's Percolator~\cite{Percolator:OSDI2010},
MongoDB~\cite{MongoDB}, TiDB~\cite{TiDB}, YugabyteDB~\cite{YugabyteDB}, MariaDB-Galera~\cite{maria-galera}, and Dgraph~\cite{dgraph}.
% Memgraph~\cite{Memgraph}, and Apache Hive~\cite{ApacheHive}.
% In Adya's formalization of \si~\cite{Adya:PhDThesis1999},
% a transaction $T$ reads versions of keys from a snapshot,
% which is associated with a \emph{start-timestamp}, taken when it starts.
% The transaction commits only if it passes a write-write conflict detection check:
% since $T$ started, no other committed transaction has written to any key that $T$ also wrote to.
% If the check fails, $T$ aborts.
% Once $T$ commits, it is assigned a \emph{commit-timestamp} and its changes become visible to all transactions that take a snapshot afterwards.
% Committed transactions writing the same key produce different versions.
% For an execution history of a database, Adya introduces version orders
% to specify a strict total order on committed versions for each key.
\si{} prevents clients from various undesired data anomalies including fractured reads, causality violations,
lost update, and long fork~\cite{AnalysingSI:JACM2018}.
% , but it allows write skew anomalies.
However, it is notoriously difficult to implement databases correctly,
with many databases failing to provide \si{} as they claim~\cite{Elle:VLDB2020, MongoDB-Jepsen, TiDB-Jepsen}.

\bfit{The SI Checking Problem.}
In this paper, we study the \si{} checking problem which asks whether a given database history satisfies \si.
\red{We address this problem via a black-box testing of \si{} in databases~\cite{FunandProfit:PODC2011},
% This is kind of dynamic analysis, different from static analysis
% which means analyzing an application program statically, without dynamically executing it~\cite{IsoDiff:VLDB2020}.
% Dynamic analysis is suitable to black-box testing of databases,
since white-box testing is often prohibitively expensive~\cite{},
restricted to specific data models~\cite{Elle:VLDB2020},
or even impossible when crucial information is unavailable~\cite{jack-clark}.}

\bfit{Challenges.} \red{TODO: integrate the challenges at the end of this section here}
The key to solving the \si{} checking problem is to resolve the \emph{uncertainties}
on the version orders between all transactions that write the same key in a history.
The challenges lie in designing an \si{} checker that is~\cite{Elle:VLDB2020}:
\begin{itemize}
  \item (Sound and Complete) It produces no \red{false positives}
    (that is, if a history fails the checker, then it indeed violates \si)
	or \red{false negatives} (that is, if a history indeed violates \si, the checker must refuse it).
	This requires a precise characterization of \si.
	Roughly speaking, a history satisfies \si{} if and only if
	there \emph{exists} a dependency graph of this history such that
	it contains only cycles of a specific pattern~\cite{AnalysingSI:JACM2018}.
	However, a dependency graph of a history represents only a single possibility of the version orders.
	How should we characterize the uncertainties on version orders
	in a single structure so that we can encode them altogether?
  \item (General) It should not be restricted to specific patterns of transactions.
    Moreover, it should not rely on specific data models of workloads or low-level system information.
  \item (\red{\it Effective}) It helps find \si{} violations in production databases.
  \item (Efficient) It is able to check histories of large sizes in reasonable time.
	A bad news is the \si{} checking problem has proven to be (in general) \npc~\cite{Complexity:OOPSLA2019}.
	Specifically, it is unrealistic to enumerate and check all possible version orders for each key
	individually in a brute-force manner.
	How to efficiently resolve the uncertainties on potential version orders
	and even better prune the impossible ones?
  \item (Informative) It should identify a violation and
	report an understandable counterexample for it when a history fails the checker.
	Such a counterexample should contain all crucial transactions
	and be kept as concise as possible.
\end{itemize}

\bfit{Related Work.}
\red{However, we are aware of no \si{} checkers that satisfy all these goals.}
Biswas and Enea proposed a polynomial-time checking algorithm
when the number of sessions is considered to be a constant~\cite{Complexity:OOPSLA2019}.
However, it is neither practically efficient
(see our performance evaluation in Section~\ref{section:experiments}) nor \red{informative}.
Although Elle is quite efficient~\cite{Elle:VLDB2020},
it relies on specific data models, e.g., lists, and/or low-level system information.
Hence, it is not general, \red{or it is not black-box at all}.
CobraSI reduces the \si{} checking problem to the \ser{} checking problem~\cite{Complexity:OOPSLA2019},
and then solves it utilizing Cobra~\cite{Cobra:OSDI2020}, a state-of-the-art serializability checker.
This approach is neither practically efficient due to the reduction procedure
(see our performance evaluation in Section~\ref{section:experiments}) nor informative due to Cobra.
Section~\ref{ss:related-work-checking-si} provides further discussion of related work.

\bfit{Contributions.}
In this work, we present \name{},
an \si{} checker satisfying all the goals mentioned above. Specifically,
\begin{itemize}
  \item We present a new (generalized-) polygraph-based characterization of \si{} (Section~\ref{section:polygraph-si}).
	A polygraph of a history can be viewed as a family of dependency graphs of this history,
	capturing all uncertainties on the version orders.
	A history satisfies \si{} if and only if its polygraph is so-called \si-acyclic.
  \item \name{} encodes the \si{} checking problem into a constraint satisfibility problem
	based on the new characterization of \si{} and solves it utilizing MonoSAT,
	an off-the-shelf SMT solver well-suited to checking graph properties such as acyclicity (Section~\ref{section:si-sat}).
    To speed up MonoSAT, \name{} prunes impossible version orders before solving.
	\red{TODO: hfwei: Compacting!!!}
  \item We evaluate \name{} in Section~\ref{section:experiments}.
    We apply \name{} to several production databases,
    and found \si{} violations in Dgraph~\cite{dgraph}, MariaDB-Galera~\cite{maria-galera}, and YugabyteDB~\cite{YugabyteDB},
	demonstrating the effectiveness of our tool.
	\name{} is also informative as it presents the witness of the \si{} violation returned by MonoSAT in an understandable way.
	Specifically, we identify the violation in MariaDB-Galera as a \emph{lost update}
	and those in Dgraph and YugabyteDB as a \emph{causality violation}.
	Finally, we compare \name's performance to other state-of-the-art tools, demonstrating its efficiency.
\end{itemize}

% Section~\ref{section:problem-definition} presents the definition and dependency graph-based characterization of \si{}
% and defines the \si{} checking problem.
% Section~\ref{section:discussion} discusses limitations and possible extensions of our approach.
% Section~\ref{section:related-work} reviews the related work.
% Section~\ref{section:conclusion} concludes.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/related-work.tex <==
% related-work.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}  \label{section:related-work}

%%%%%%%%%%%%%%%
\subsection{Characterizing Snapshot Isolation}	\label{ss:si}

There are numerous variants of snapshot isolation in the literature~\cite{ClientCentric:PODC2017},
such as Adya \si~\cite{Adya:PhDThesis1999}, ANSI \si~\cite{CritiqueANSI:SIGMOD1995},
PSI (Parallel \si)~\cite{PSI:SOSP2011}, GSI (Generalized \si)~\cite{GSI:SRDS2005},
Strong Session \si~\cite{AnalysingSI:JACM2018, LazyReplSI:VLDB2006}, Strong \si~\cite{LazyReplSI:VLDB2006},
NMSI (Non-Monotonic \si)~\cite{NMSI:SRDS2013}, and so on.
In this work, we use the Strong Session variant of \si.

Several ways have been proposed to characterize (the variants of) snapshot isolation
(and other isolation levels).
\si{} was first defined in ~\cite{CritiqueANSI:SIGMOD1995}
by a multi-version concurrency control algorithm as described in Section~\ref{ss:si-informal}.
% In~\cite{CritiqueANSI:SIGMOD1995}, \si{} was also (informally) characterized by the write skew anomaly that it allowed.
Adya~\cite{Adya:PhDThesis1999} presented an implementation-independent specification
of \si{} in terms of dependency graphs.
% It was shown that a history satisfies \si{} if and only if G1 and G-SI anomalies are disallowed,
% where G1 and G-SI anomalies are defined as certain bad patterns in dependency graphs.
However, as pointed out by Cerone and Gotsman in~\cite{AnalysingSI:JACM2018},
the dependency graphs used in~\cite{Adya:PhDThesis1999} still contain the low-level \emph{start-dependency} relation
which captures the system's choice of ordering start and commit events of transactions.
Recently, Cerone et al. proposed an axiomatic $(\vis, \ar)$ framework for specifying a variety of transactional
consistency models uniformly and declaratively~\cite{Framework:CONCUR2015}.
% To declaratively describe how the system process transactions, they extend histories with two relations:
% the visibility relation $\vis$ captures the set of transactions that each transaction can observe,
% and the arbitration relation $\ar$ specifies the version orders for each key.
Based on the $(\vis, \ar)$ framework,
Cerone and Gotsman proposed the first characterization of \si{} solely in terms of dependency graphs
\emph{without} using the start-dependency relation~\cite{AnalysingSI:JACM2018}.
We use this characterization (repeated in Theorem~\ref{thm:polygraph-si}) as the theoretical foundation of our \si{} checking algorithm.
Furthermore, to capture all uncertainties on the version orders for each key in a history
in a single structure instead of in multiple separate dependency graphs,
we propose a new (generalized-) polygraph-based characterization of \si.

% Crooks et al. introduced a client-centric state-based axiomatic formalization of transactional consistency models,
% and used it to organize several variants of \si{} in a clean hierarchy~\cite{ClientCentric:PODC2017}.
% Xiong et al. provided a state-based interleaving operational semantics for distributed atomic transactions,
% and used it to prove the correctness of the Clock-SI protocol
% for partitioned key-value stores~\cite{ClockSI:SRDS2013} which satisfies \si~\cite{CentralisedSemantics:ECOOP2020}.
%%%%%%%%%%%%%%%
\subsection{Transactional Consistency Checking: Dynamic Analysis} \label{ss:tcc-dynamic}

In terms of dynamic analysis, transactional consistency checking means
dynamically executing a database and checking whether the histories
it generates satisfy some consistency model.
Biswas and Enea showed that consistency models like RC, RA, and TCC are polynomial-time checkable
while \si{} and \ser{} are \npc{} in general,
namely, when the version orders for each key are unknown~\cite{Complexity:OOPSLA2019}.
They devised a polynomial-time algorithm for checking \ser{}
when the number of sessions is considered to be a constant.
By reducing the \si{} checking problem to \ser{} in polynomial time,
they also obtained a polynomial-time algorithm for checking \si.
However, this algorithm is neither informative nor as practically efficient as \name.

Elle~\cite{Elle:VLDB2020} is highly efficient in checking a variety of consistency models
and has found many violations in production databases~\cite{Elle:VLDB2020}.
To this end, Elle relies on specific data models, e.g., lists, in workloads
to infer the version orders from histories.
In contrast, \name{} uses only the common key-value APIs and are more generally applicable.
Even more problematic, Elle relies on the start and commit timestamps of transactions,
which may not be exposed to clients, to infer the start-dependency relation
used in Adya's dependency graph-based characterization of \si.

Cobra made use of the dependency graph-based characterization of \ser{}
to reduce the \ser{} checking problem into a constraint satisfibility problem
and feed it to the MonoSAT solver~\cite{Cobra:OSDI2020}.
A history satisfies \ser{} if and only if the history has an acyclic dependency graph.
In this work, we exploit the dependency graph-based characterization of \si{} in~\cite{AnalysingSI:JACM2018}.
Compared to that of \ser,
the characterization of \si{} is defined on a more complex cycle pattern in dependency graphs.
It is thus more challenging to make \name{} effective and efficient in both constraints pruning and MonoSAT encoding.
Morevoer, compared to Cobra, \name{} is informative as it can present the witness of the \si{} violation returned by MonoSAT in an understandable way.

% Liu et al. conducted a fully automated white-box checking of distributed transaction systems
% described in Maude~\cite{AllAboutMaude:Book2007} against nine common transactional consistency models~\cite{Maude:Liu2019}.
% This is based on automatically recording relevant history during a Maude run and
% defining the consistency properties on such histories.
The anomaly detector tool ConsAD enforces a commit order for update transactions to infer $\WW$ edges
by serializing them via exclusively updating an artificial shared variable~\cite{ConsAD:VLDB2014}.
Furthermore, ConsAD quantifies anomalies by finding all cycles occurred in the dependency graph of a history.
RushMon demonstrates that the number of cycles in the dependency graph
is a good indicator of the system ``chaos''~\cite{RushMon:SIGMOD2018}.
We do not quantify anomalies in this work.
%%%%%%%%%%%%%%%
\subsection{Transactional Consistency Checking: Static Analysis} \label{ss:tcc-static}

In terms of static analysis, transactional consistency checking means
analyzing an application program statically, without dynamically executing it.
Compared to dynamic analysis, static analysis is able to locate the root causes
of anomalies in application programs.

By static analysis, Fekete studied the problem of
allocating separate isolation levels such as \si{} and \ser{} to each transaction in a program,
while still ensuring that every execution will be conflict serializable~\cite{AllocatingIsolation:PODS2005}.
Jorwekar et al. developed a syntactic analysis technique to automatically
identify all the transactions that could cause \si{} violations
among a given set of transactions~\cite{DetectionSI:VLDB2007}.
Warszawski and Bailis defined the problem of ACIDRain attacks
and developed 2AD (Abstract Anomaly Detection),
a dynamic analysis tool that uses traces of normal database activity
to detect possible anomalies in applications~\cite{ACIDRain:SIGMOD2017}.
Gan et al. proposed the tool IsoDiff to help developers debug anomalies
caused by weak isolation levels, including RC and \si, for application programs~\cite{IsoDiff:VLDB2020}.
% IsoDiff first builds a dependency graph with all possible dependency edges by analyzing the program
% and then searches for certain types of cycles in the dependency graph.
For the purpose of debugging, they reduced both false negatives and false positives.
% Fekete et al. quantified isolation anomalies by defining a novel microbenchmark
% that measures how rapidly integrity violations are produced at different isolation levels,
% for a simple set of transactions~\cite{QuantifyingAnomalies:VLDB2009}.
%%%%%%%%%%%%%%%
%\subsection{Robustness against Transactional Consistency Models} \label{ss:robustness}


% Robustness against consistency models with atomic visibility~\cite{Robustness:CONCUR2016},
% Robustness against snapshot isolation~\cite{RobustnessSI:CAV2019},
% Robustness against lower isolation levels~\cite{RobustnessLower:PODS2020}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/so_combine_prove.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Here is the  of prove of cut counterexample
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{algs/clip-counterexample}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Here is the start of prove of cut counterexample
%%%%%%%%%%%%%%%%%%%%%%%%%%%


%soundness of the first step
%completeness is not satisfied
\begin{lemma}[First step of reduce cycle]
    \label{lemma:ce-dgraph}
    History $H$ has a cycle $C$, which means $H$ do not meat $SI$.
    $C$ can be cut into a small cycle $C'$ by a $\rel{so}$,
    then $C'$ represents a behavior of $H$ against $SI$.
\end{lemma}

\begin{proof}
    \label{proof:ce-dgraph}
    For a history, a cycle means that the history do not satisfy $SI$.
    Though a new `so' edge is inserted to cut the $C$ into $C'$,
    the new `so' edge actually exists in the history.
    Thus, $C'$ exists objectively in $H$, 
    and represents true behaviors that violate $SI$ as well.
\end{proof}

\begin{lemma}
    \label{lemma:so-combine-1}
    History $H$ has a minimal cycle $C$ of size larger than 4,
    in which each session has at most two adjacent transactions.
    For any two adjacent transactions $t_1\rel{so}t_2$ in $C$,
    there will not be a transaction $t_3$ in $C$, 
    which is linked to an edge with $t_1$ and another edge with $t_2$.
\end{lemma}

\begin{proof}
    \label{proof:so-combine-1}
    If there exists $t_3$, then there will be four cases:
    
    1.($t_1->t_3$)\&($t_2->t_3$), 
    
    2.($t_1->t_3$)\&($t_3->t_2$),
    
    3.($t_3->t_1$)\&($t_2->t_3$),
    
    4.($t_3->t_1$)\&($t_3->t_2$).
    
    case 1:
    
    In this case, there will be a small cycle ($t_1->t_3$)+$C_{t_3->t_1}$. 
    Here $C_{t_3->t_1}$ is the path from $t_3$ to $t_1$ in $C$.
    
    case 2:
    
    In this case, there will be a small cycle ($t_3->t_2$)+$C_{t_2->t_3}$. 
    Here $C_{t_2->t_3}$ is the path from $t_2$ to $t_3$ in $C$.
    
    case 3:
    
    In this case, there will be a small cycle 
    ($t_3->t_1$)+($t_2->t_1$)+($t_1->t_2$). 
    
    case 4:
    
    In this case, there will be a small cycle 
    ($t_3->t_2$)+$C_{t_2->t_3}$. 
    Here $C_{t_2->t_3}$ is the path from $t_2$ to $t_3$ in $C$.
\end{proof}

\begin{lemma}
    \label{lemma:combine-dependency(k)}
    History $H$ has a minimal cycle $C$ of size larger than 4,
    in which each session has at most two adjacent transactions.
    
    For any two adjacent transactions $t_1\rel{so}t_2$ in $C$,
    and there exists a dependency $t_1\rel{wr(k)/ww(k)/rw(k)}t_2$. 
    We move all the operations about key $k$ in $t_2$ into $t_1$.
    We keep that $(operations$ $in$ $t_1)\rel{po}(operations$ $moved$ $from$ $t_2)$ in $t_1$ and make a new $t_1' \rel{} t_2'$.
    
    After our change, we came to this conclusion:
    
    For any dependency $t_x\rel{}t_y$, ($t_x \neq t_1/t_2$ or $t_y \neq t_1/t_2$),  it will still be kept after our change.
\end{lemma}

\begin{proof}
    For a dependency $t_x\rel{}t_y$, there are the following 4 cases:
    
    case1: $t_x \neq t_1$, $t_x \neq t_2$, $t_y \neq t_1$, $t_y \neq t_2$.
    
    In this case, there is no relationship between $t_x\rel{}t_y$ and $t_1\rel{}t_2$. Whatever we change between $t_1$ and $t_2$ will not affect $t_x\rel{}t_y$.
    
    case2: $t_x\rel{wr(k')/ww(k')/rw(k')}t_y$, $k \neq k'$.
    
    In this case, $t_x\rel{op(k')}t_y$ and $t_1\rel{op(k)}t_2$ associated with two different keys. So whatever we do with operations about key $k$ will not affect $t_x\rel{op{k'}}t_y$.
    
    case3: $t_x \neq t_1$, $t_x \neq t_2$, $t_y = t_1$. $t_x\rel{op(k)}t_y$.
    
    In this case, $t_x\rel{}t_1$ and $t_1\rel{}t_2$ are associated with the same key $k$. 
    Here we know that there will not be a dependency
    $t_2->t_x$ (lemma~\ref{lemma:so-combine-1}). 
    So there is a strict total order between the three transactions:
    $t_x\rel{}t_1\rel{}t_2$. 
    In our construction, we move the operations in $t_2$ into $t_1$,
    and keep a program order in $t_1$: $(operaions in t_1)\rel{po}(operations moved from t_2)$.
    The dependency $t_x\rel{}t_1$ will trivially be still kept.
    
    case4: $t_x = t_2$, $t_y \neq t_1$, $t_y \neq t_2$. $t_x\rel{op(k)}t_y$.
    
    In this case, $t_1\rel{}t_2\rel{}t_y$ and 
    the two dependencies are associated with the same key $k$.
    We know that there will not be a dependency $t_y\rel{}t_1$(lemma~\ref{lemma:so-combine-1}).
    So there is a strict total order between the three transactions:
    $t_1\rel{}t_2\rel{}t_y$.
    In our construction, we move all the operations 
    associated with $k$ in $t_2$ into $t_1$.
    Thus we have this order: $(ops$ $in$ $t_1)\rel{po}(ops$ $moved$ $from$ $t_2)$ $\rel{}t_y$. 
    Notice here $t_2\rel{}t_y$ is changed into $t_1\rel{}t_y$.
    But once we move all operations in $t_2$ into $t_1$, 
    then $t_2$ and $t_1$ will be combined into one transaction $t_1':[t_1 \rel{po} t_2]$.
    Thus $(t_1':[t_1 \rel{po} t_2])\rel{}t_y$ still keeps the
    information of $t_2\rel{}t_y$.
\end{proof}

\begin{lemma}
    \label{lemma:so-combine-2}
    History $H$ has a minimal cycle $C$ of size larger than 4,
    in which each session has at most two adjacent transactions.
    For any two adjacent transactions $t_1\rel{so}t_2$ in $C$,
    combine them into one transaction will not change the information in the cycle.
\end{lemma}

\begin{proof}
    \label{proof:so-combine-2}
    For $t_1\rel{op(k)}t_2$, move all operations associated with key $k$ in $t_2$ into $t_1$ will do nothing with other dependencies in $C$(lemma~\ref{lemma:combine-dependency(k)}).
    
    After moving all those operations in $t_2$ into $t_1$, 
    the left operations in $t_2$ have no relationships with operations
    in $t_1$. Move them into $t_1$ will make no impact.
    
    Thus, combine $t_1$ and $t_2$ into $t_1':[t_1\rel{po}t_2]$ will
    not change any information of the cycle.
\end{proof}

==> tables/_region_.tex <==
\message{ !name(memory.tex)}
\message{ !name(memory.tex) !offset(116) }
\begin{axis}[
					x tick style={draw=none},
					x tick label style={rotate=45,anchor=east},
					ylabel={Memory (MiB)},
					ymin=0,
					ybar,
					bar width=7,
					area legend,
					legend pos=north east,
					xtick=data,
					xticklabels={RUBiS,TPC-C,C-Twitter,GeneralRH,GeneralRW,GeneralWH}
				]
				\addplot[fill=white] table [x expr=\coordindex, y=cobra, col sep=comma] {tables/data/memory-cobra-10k-compare.csv};
				\addplot[pattern=north east lines] table [x expr=\coordindex, y=si, col sep=comma] {tables/data/memory-cobra-10k-compare.csv};
				\legend{Cobra w/ GPU,\name}
			\end{axis}
\message{ !name(memory.tex) !offset(-19) }


==> tables/comparison.tex <==
% comparison.tex

% \usepackage{graphicx}
\begin{table}[t]
  \centering
  \caption{Comparison}
  \label{table:comparison}
  \resizebox{0.45\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|}
      \hline
                  & OOPSLA & Elle &  Cobra (\ser) &  &  \\ \hline
      Sound       &        & \yes &  \yes &  &  \\ \hline
      Complete    &        & \no  &  \yes &  &  \\ \hline
      Effective   &        &      &  &  &  \\ \hline
      Informative &        &      &  &  &  \\ \hline
      General     &        &      &  \yes &  &  \\ \hline
      Efficiency  &        &      &  &  &  \\ \hline
      Online  	  &   &      &  &  &  \\ \hline
      Full-featured  &        &      &  &  &  \\ \hline
    \end{tabular}%
}
\end{table}


==> tables/table-axioms.tex <==
% table-axioms.tex

\begin{table*}[t]
  \centering
  \caption{Consistency axioms, constraining an abstract execution $(\h, \vis, \ar)$.
    (From~\protect\cite{JACM2018:AnalysingSI})}
  \label{table:axioms}
  \renewcommand{\arraystretch}{1.8}
  \resizebox{0.80\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{
	  $\begin{aligned}[c]
		&\forall (\E, \po) \in \h.\;
		  \forall \evar \in \Event.\;
		    \forall \keyxvar, \valvar.\;
			  \big(\op(\evar) = \readevent(\keyxvar, \valvar)
			  \land \set{\fvar \mid \op(\fvar) = \_(\keyxvar, \_) \land \fvar \rel{\po} \evar} \neq \emptyset\big) \\
			  &\quad \implies \op(\max_{\po} \set{\fvar \mid \op(\fvar) = \_(\keyxvar, \_) \land \fvar \rel{\po} \evar}) = \_(\keyxvar, \valvar)
	   \end{aligned}$ \hfill (\intaxiom)} \\ \hline
    \multicolumn{4}{|c|}{
	  $\begin{aligned}[c]
		\forall T \in \h.\; \forall \keyxvar, \valvar.\; T \vdash \readevent(\keyxvar, \valvar) \implies
		  \max_{\ar}(\vis^{-1}(T) \cap \WriteTx_{\keyxvar}) \vdash \writeevent(\keyxvar, \valvar)
	  \end{aligned}$ \hfill (\extaxiom)} \\ \hline
    $\SO \subseteq \vis$ \hfill (\sessionaxiom)
	& $\ar \comp \vis \subseteq \vis$ \hfill (\prefixaxiom)
	& \multicolumn{2}{c|}{$\forall S, T \in \h.\; S \conflict T \implies (S \rel{\vis} T \lor T \rel{\vis} S)$
	  \hfill (\noconflictaxiom)} \\ \hline
    \end{tabular}%
  }
\end{table*}
